Identifying systemically important companies in the entire liability network of a small open economy

To a large extent, the systemic importance of financial institutions is related to the topology of financial liability networks. In this work we reconstruct and analyze the - to our knowledge - largest financial network that has been studied up to now. This financial liability network consists of 51,980 firms and 796 banks. It represents 80.2% of total liabilities towards banks by firms and all interbank liabilities from the entire Austrian banking system. We find that firms contribute to systemic risk in similar ways as banks do. In particular, we identify several medium-sized banks and firms with total assets below 1 bln. EUR that are systemically important in the entire financial network. We show that the notion of systemically important financial institutions (SIFIs) or global and domestic systemically important banks (G-SIBs or D-SIBs) can be straightforwardly extended to firms. We find that firms introduce slightly more systemic risk than banks. In Austria in 2008, the total systemic risk of the interbank network amounts to only 29% of the total systemic risk of the entire financial network, consisting of firms and banks.

==> img/hists/hist.tex <==
% !TeX root = ../../MSc.tex

==> img/hists/histBud.tex <==
% !TeX root = ../../MSc.tex
\begin{tikzpicture}
	\def\dB{./data/5000c/hists/BDeg4.csv}
	\def\dIB{./data/5000c/hists/IBDeg4.csv}
	\def\dBx{./data/5000c/hists/BDeg3.csv} % range up to 5k
	\def\dIBx{./data/5000c/hists/IBDeg3.csv} % uses same range as BDeg2 instead of reduced range
	\begin{axis}[
		,	width=0.95\textwidth
		,	height=170pt
		%,	axis on top
		,	scale only axis
		,	ymode=log
		%,	xmode=log
		,	ybar = 0pt% -3pt
		,	legend cell align = left
		,	bar width= 3.75pt
		%,	x tick label as interval=false
		%,	xtickten={-16,-14,-12,...,4}
		%,	yticklabel={}
		,	xtick pos=left
		,	ytick pos=left
		,	xmin=-60
		,	xmax=5000
		,	ymin=0.5
		,	ymax=1000
		%,	grid=none
		,	ymajorgrids
		,	log origin=infty
		,	cycle list name=compBankList
		,	ylabel = {Count}
		,	xlabel = {Undirected degrees of banks}
		,	ylabel near ticks]
		\addplot+[,draw=none] table [x=left,y=undirected] {\dBx};
		\addplot+[,draw=none] table [x=left,y=undirected] {\dIBx};
	\end{axis}
	\begin{axis}[
		,	width=0.79\textwidth
		,	xshift=2.6cm
		,	yshift=1.6cm
		,	height=120pt
		,				,	axis background/.style={fill=gray!02}
		,	scale only axis
		,	ymode=log
		%,	xmode=log
		,	ybar = 0pt% -3pt
		,	legend cell align = left
		,	legend style={draw=none}
		,	bar width= 2pt
		%,	x tick label as interval=false
		%,	xtickten={-16,-14,-12,...,4}
		%,	yticklabel={}
		,	xtick pos=left
		,	ytick pos=left
		,	xmin=-10
		,	xmax=600
		,	ymin=0.5
		%,	ymax=1
		%,	grid=none
		,	ymajorgrids
		,	log origin=infty
		,	cycle list name=compBankList
		,	ylabel = {Count}
		,	xlabel = {Undirected degrees of banks}
		,	ylabel near ticks
		,	ylabel style={fill = white}
		]
		\addplot+[,draw=none] table [x=left,y=undirected] {\dB};\addlegendentry{Full network}\label{plt:deg:f}
		\addplot+[,draw=none] table [x=left,y=undirected] {\dIB};\addlegendentry{Interbank network}\label{plt:deg:ib}
	\end{axis}
\end{tikzpicture}

==> img/histsT/hist.tex <==
% !TeX root = ../../MSc.tex

==> img/histsT/histBF.tex <==
% !TeX root = ../../MSc.tex
\begin{tikzpicture}
	\def\DRTX{./data/5000c/hists/BDeg.csv}
	\def\DRT{./data/5000c/hists/BDeg2.csv}
	\begin{axis}[
		,	width=0.95\textwidth
		,	height=170pt
		%,	axis on top
		,	scale only axis
		,	ymode=log
		%,	xmode=log
		,	ybar = 0pt% -3pt
		,	legend cell align = left
		,	bar width= 3pt
		%,	x tick label as interval=false
		%,	xtickten={-16,-14,-12,...,4}
		%,	yticklabel={}
		,	xtick pos=left
		,	ytick pos=left
		,	xmin=-40
		,	xmax=2600
		,	ymin=0.5
		,	ymax=1000
		%,	grid=none
		,	ymajorgrids
		,	log origin=infty
		,	cycle list name=compBankList
		,	ylabel = {Count}
		,	xlabel = {Degree of banks in full network}
		,	ylabel near ticks
		]
		\addplot+[,draw=none] table [x=left,y=in] {\DRT};
		\addplot+[,draw=none] table [x=left,y=out] {\DRT};
	\end{axis}
	\begin{axis}[
		,	width=0.75\textwidth
		,	xshift=2.6cm
		,	yshift=2.1cm
		,	height=105pt
		,				,	axis background/.style={fill=gray!02}
		,	scale only axis
		,	ymode=log
		%,	xmode=log
		,	ybar = 0pt% -3pt
		,	legend cell align = left
		,	legend style={draw=none}
		,	bar width= 1.25pt
		%,	x tick label as interval=false
		%,	xtickten={-16,-14,-12,...,4}
		%,	yticklabel={}
		,	xtick pos=left
		,	ytick pos=left
		,	xmin=-1
		,	xmax=100
		,	ymin=0.5
		%,	ymax=1
		%,	grid=none
		,	ymajorgrids
		,	log origin=infty
		,	cycle list name=compBankList
		,	ylabel = {Count}
		,	xlabel = {Degree of banks in full network}
		,	ylabel near ticks
		,	ylabel style={fill = white}
		]
		\addplot+[,draw=none] table [x=left,y=in] {\DRTX};\addlegendentry{Indegree}
		\addplot+[,draw=none] table [x=left,y=out] {\DRTX};\addlegendentry{Outdegree}
	\end{axis}
\end{tikzpicture}

==> img/histsT/histBIB.tex <==
% !TeX root = ../../MSc.tex
\begin{tikzpicture}
	\def\DRTX{./data/5000c/hists/IBDeg.csv}
	\def\DRT{./data/5000c/hists/IBDeg2.csv}
	\begin{axis}[
		,	width=0.95\textwidth
		,	height=170pt
		%,	axis on top
		,	scale only axis
		,	ymode=log
		%,	xmode=log
		,	ybar = 0pt% -3pt
		,	legend cell align = left
		,	bar width= 3pt
		%,	x tick label as interval=false
		%,	xtickten={-16,-14,-12,...,4}
		%,	yticklabel={}
		,	xtick pos=left
		,	ytick pos=left
		,	xmin=-5
		,	xmax=360
		,	ymin=0.5
		,	ymax=2000
		%,	grid=none
		,	ymajorgrids
		,	log origin=infty
		,	cycle list name=compBankList
		,	ylabel = {Count}
		,	xlabel = {Degree of banks in interbank network}
		,	ylabel near ticks
		]
		\addplot+[,draw=none] table [x=left,y=in] {\DRT};
		\addplot+[,draw=none] table [x=left,y=out] {\DRT};
	\end{axis}
	\begin{axis}[
		,	width=0.75\textwidth
		,	xshift=2.6cm
		,	yshift=2.6cm
		,	height=90pt
		,				,	axis background/.style={fill=gray!02}
		,	scale only axis
		,	ymode=log
		%,	xmode=log
		,	ybar = 0pt% -3pt
		,	legend cell align = left
		,	legend style={draw=none}
		,	bar width= 1.25pt
		%,	x tick label as interval=false
		%,	xtickten={-16,-14,-12,...,4}
		%,	yticklabel={}
		,	xtick pos=left
		,	ytick pos=left
		,	xmin=-1
		,	xmax=100
		,	ymin=0.5
		,	ymax=1000
		%,	grid=none
		,	ymajorgrids
		,	log origin=infty
		,	cycle list name=compBankList
		,	ylabel = {Count}
		,	xlabel = {Degree of banks in interbank network}
		,	ylabel near ticks
		,	ylabel style={fill = white, xshift = 1cm}
		]
		\addplot+[,draw=none] table [x=left,y=in] {\DRTX};\addlegendentry{Indegree}
		\addplot+[,draw=none] table [x=left,y=out] {\DRTX};\addlegendentry{Outdegree}
	\end{axis}
\end{tikzpicture}

==> img/histsT/histBud.tex <==
% !TeX root = ../../MSc.tex
\begin{tikzpicture}
	\def\dB{./data/5000c/hists/BDeg4.csv}
	\def\dIB{./data/5000c/hists/IBDeg4.csv}
	\def\dBx{./data/5000c/hists/BDeg3.csv} % range up to 5k
	\def\dIBx{./data/5000c/hists/IBDeg3.csv} % uses same range as BDeg2 instead of reduced range
	\begin{axis}[
		,	width=0.95\textwidth
		,	height=170pt
		%,	axis on top
		,	scale only axis
		,	ymode=log
		%,	xmode=log
		,	ybar = 0pt% -3pt
		,	legend cell align = left
		,	bar width= 3pt
		%,	x tick label as interval=false
		%,	xtickten={-16,-14,-12,...,4}
		%,	yticklabel={}
		,	xtick pos=left
		,	ytick pos=left
		,	xmin=-60
		,	xmax=5000
		,	ymin=0.5
		,	ymax=1000
		%,	grid=none
		,	ymajorgrids
		,	log origin=infty
		,	cycle list name=compBankList
		,	ylabel = {Count}
		,	xlabel = {Undirected degrees of banks}
		,	ylabel near ticks]
		\addplot+[,draw=none] table [x=left,y=undirected] {\dBx};
		\addplot+[,draw=none] table [x=left,y=undirected] {\dIBx};
	\end{axis}
	\begin{axis}[
		,	width=0.75\textwidth
		,	xshift=2.6cm
		,	yshift=1.6cm
		,	height=120pt
		,				,	axis background/.style={fill=gray!02}
		,	scale only axis
		,	ymode=log
		%,	xmode=log
		,	ybar = 0pt% -3pt
		,	legend cell align = left
		,	legend style={draw=none}
		,	bar width= 1.5pt
		%,	x tick label as interval=false
		%,	xtickten={-16,-14,-12,...,4}
		%,	yticklabel={}
		,	xtick pos=left
		,	ytick pos=left
		,	xmin=-10
		,	xmax=600
		,	ymin=0.5
		%,	ymax=1
		%,	grid=none
		,	ymajorgrids
		,	log origin=infty
		,	cycle list name=compBankList
		,	ylabel = {Count}
		,	xlabel = {Undirected degrees of banks}
		,	ylabel near ticks
		,	ylabel style={fill = white}
		]
		\addplot+[,draw=none] table [x=left,y=undirected] {\dB};\addlegendentry{Full network}\label{plt:deg:f}
		\addplot+[,draw=none] table [x=left,y=undirected] {\dIB};\addlegendentry{Interbank network}\label{plt:deg:ib}
	\end{axis}
\end{tikzpicture}

==> img/histsT/histC.tex <==
% !TeX root = ../../MSc.tex
\begin{tikzpicture}
	\def\DRT{./data/5000c/hists/CDeg.csv}
	\begin{axis}[
		,	width=0.35\textwidth
		,	height=100pt
		%,	axis on top
		,	scale only axis
		,	ymode=log
		%,	xmode=log
		,	ybar = 0pt% -3pt
		,	legend cell align = left
		,	bar width= 4pt
		,	legend style={draw=none}
		,	xtick pos=left
		,	ytick pos=left
		,	xmin=0
		%,	xmax=0.7
		,	ymin=1
		,	ymax=4000
		%,	grid=none
		,	ymajorgrids
		,	log origin=infty
		,	cycle list name=compBankList
		,	ylabel = {Count}
		,	xlabel = {Degree of companies in full network}
		]
		\addplot+[,draw=none] table [x=left,y=in] {\DRT};\addlegendentry{Indegree}
		\addplot+[,draw=none] table [x=left,y=out] {\DRT};\addlegendentry{Outdegree}
	\end{axis}
\end{tikzpicture}  

==> img/histsT/histDR.tex <==
% !TeX root = ../../MSc.tex
\begin{tikzpicture}
	\def\DRT{./data/5000c/hists/DR.csv}
	\begin{axis}[
		,	width=0.9\textwidth
		,	height=170pt
		%,	axis on top
		,	scale only axis
		,	ymode=log
		,	ybar
		,	legend cell align = left
		%,	bar width= 3.75pt
		%,	x tick label as interval=false
		,	xtick={0,0.1,0.2,0.3,0.4,0.5,0.6,0.7}
		%,	yticklabel={}
		,	xtick pos=left
		,	ytick pos=left
		,	xmin=-0.015
		,	xmax=0.7
		,	ymin=0.5
		%,	ymax=1
		%,	grid=none
		,	ymajorgrids
		,	log origin=infty
		,	cycle list name=compBankList
		,	ylabel = Count
		,	xlabel = DebtRank $R^F$
		,	ylabel near ticks
		]
		\addplot+[bar width=4pt] table [x=left,y=c] {\DRT};\label{plt:drhist:companies}%\addlegendentry{Companies}
		%				\addplot+[bar width=2.25pt,draw=none] table [x=left,y=b] {\DRT};%\addlegendentry{Banks}
		
	\end{axis}
	\begin{axis}[
		,	width=0.7\textwidth
		,	xshift = 2.5cm
		,	yshift = 2.34cm
		,	axis background/.style={fill=gray!02}
		,	height=100pt
		%,	axis on top
		,	scale only axis
		,	ymode=log
		,	ybar = -3.15pt
		,	legend cell align = left
		,	bar width= 3.15pt
		,	xtick={0,0.1,0.2,0.3,0.4,0.5,0.6,0.7}
		,	xtick pos=left
		,	ytick pos=left
		,	xmin=-0.015
		,	xmax=0.7
		,	ymin=0.5
		%,	ymax=1
		%,	grid=none
		,	ymajorgrids
		,	log origin=infty
		,	cycle list name=compBankList
		,	ylabel = Count
		,	xlabel = DebtRank $R^F$
		,	ylabel near ticks
%		,	ylabel style = {fill = white}
		,	legend style={fill=white, fill opacity=0.9, draw opacity=1,text opacity=1, draw = none}
		]

		% Combined legend for two plots - use refstyle
		\addlegendimage{/pgfplots/refstyle=plt:drhist:companies}\addlegendentry{Companies}
		\addplot[bankColor] table [x=left,y=b] {\DRT};\label{plt:drhist:banks}
		\addlegendimage{/pgfplots/refstyle=plt:drhist:banks}\addlegendentry{Banks}
		
	\end{axis}
\end{tikzpicture}
